Word Sense Disambiguation in Native Spanish: A Comprehensive Lexical Evaluation Resource

Human language, while aimed at conveying meaning, inherently carries ambiguity. It poses challenges for speech and language processing, but also serves crucial communicative functions. Efficiently solve ambiguity is both a desired and a necessary characteristic. The lexical meaning of a word in context can be determined automatically by Word Sense Disambiguation (WSD) algorithms that rely on external knowledge often limited and biased toward English. When adapting content to other languages, automated translations are frequently inaccurate and a high degree of expert human validation is necessary to ensure both accuracy and understanding. The current study addresses previous limitations by introducing a new resource for Spanish WSD. It includes a sense inventory and a lexical dataset sourced from the Diccionario de la Lengua Espa\~nola which is maintained by the Real Academia Espa\~nola. We also review current resources for Spanish and report metrics on them by a state-of-the-art system.

==> results_analysis.tex <==
%\appendix
%\section{Real world data normalized}
%\label{sec:appendix-evaluated-model}

\begin{table*}[!htbp]
\centering
{
\tabcolsep=0.15cm
\small
\begin{NiceTabular}{c|cccccc}[colortbl-like]	
	%\begin{center}
		%\begin{tabular}{l|c|c|c|c|r}
            \toprule

             Model  & SemEval-13 &  SemEval-15 & DLE-Eval\\
             	
                \midrule
                
			\rowcolor{gray!15}SDS & 63.71 & 68.72 & 73.89 (73.88) \\
	        
			MuLaN & 76.35 & 74.33 & 44.01(43.99) \\
   
			\rowcolor{gray!15} SemCor(SC) & 82.06 &  (77.22) & 55.48(55.47)\\

                MuLaN-SC & 78.44 & 74.91 & 41.29(41.29) \\

            \rowcolor{gray!15} SC-SDS & \textbf{83.83} & \textbf{79.00} & \textbf{73.97 (73.95)} \\

                        MuLaN- SDS & 82.02 & 77.83 & 48.31(48.29) \\


            
                \bottomrule
			
			
            %\bottomrule
		%\end{tabular}
	%\end{center}
\end{NiceTabular}}
  {\caption{F1-score(\%) of different models combining MuLan, SemCor(SC) and SDS in SE-13,  SE-15 and DLE-Eval benchmarks. For the DLE-Eval, we performed the micro and macro(in parenthesis) average F1-score. The model names are derived from the datasets employed in their respective training processes.}\label{table:results_analysis}}}


  
\end{table*}


==> table_previous_spanish_models.tex <==
%\appendix
%\section{Real world data normalized}
%\label{sec:appendix-evaluated-model}

\begin{table}[!hb]

\tabcolsep=0.20cm
\small
\begin{NiceTabular}{c|cccccc}[colortbl-like]	
	%\begin{center}
		%\begin{tabular}{l|c|c|c|c|r}
            \toprule

             Model  & SemEval-13 &  SemEval-15 \\
                \midrule
			%\rowcolor{gray!15}  ONESEC \diamondsuit & 72.0 & 62.8\\
	        
			%mBERT-CLS (Trans) \star & 70.32 & 57.62\\
   
			\rowcolor{gray!15}  mBERT-UNI (Trans) \star & 69.68 & 67.11 \\

            WNG+SyntagNet \bullet & 73.4 & 61.2 \\

            \rowcolor{gray!15}  AMuSE-WSD \bigtriangleup & 80.0 & \textbf{73.0} \\

            SensEMBERT  \spadesuit & 74.6 & 64.1 \\
            \rowcolor{gray!15} Multimirror \heartsuit  & \textbf{82.17}  & 70.42 \\
            
                \bottomrule
			
			
            %\bottomrule
		%\end{tabular}
	%\end{center}
\end{NiceTabular}
  {\caption{F1-score(\%) of many models  evaluated in  SE13 and SE15 in Spanish.
  Reported systems:
 %$\diamondsuit$ \cite{scarlini-etal-2020-sense}, 
 $\star$  \citep{su-etal-2022-multilingual}, 
 $\bullet$ \citep{maru-etal-2019-syntagnet},
 $\bigtriangleup$ \citep{orlando-etal-2021-amuse} , 
 $\spadesuit$ \citep{Scarlini_Pasini_Navigli_2020}, 
 $\heartsuit$ \citep{ijcai2021p539}.
}\label{table:table_previous_spanish}}
\end{table}

%/ \protect\cite{scarlini-etal-2020-sense}
%/ \citep{su-etal-2022-multilingual}
%/\citep{orlando-etal-2021-amuse}
%/\citep{orlando-etal-2021-amuse}, \citep{Scarlini_Pasini_Navigli_2020},\citep{ijcai2021p539}

==> table_taza.tex <==
%\appendix
%\section{Real world data normalized}
%\label{sec:appendix-evaluated-model}

\begin{table}[!tbp]

\tabcolsep=0.08cm
\small
\begin{NiceTabular}{c|c}[colortbl-like]	
	%\begin{center}
		%\begin{tabular}{l|c|c|c|c|r}
            \toprule

               \multicolumn{2}{l}{Example in   CSV}  
                \midrule
                \rowcolor{gray!15} Context       & Una {[}TGT{]}   taza {[}TGT{]}  de caldo  \\
                Lemma         &  Taza    \\
                Definition\_1 & Vasija   pequeña, por lo común de loza o de metal y   con asa, empleada generalmente   para   tomar líquidos. \\
            Definition\_2 & Cantidad   que   cabe en una taza.  \\                                                                  

   
        

                \bottomrule
			
			
            %\bottomrule
		%\end{tabular}
	%\end{center}
\end{NiceTabular}
  {\caption{Comparison between SemEval-2013 and  SemEval-2015 in the wn split. Here it is showed the amount of Instances, Word Types(WP), Word Average Polysemy (WAP),  Instance Average Polysemy(IAP),Polysemous Words(PW).}\label{table:table_taza}}
\end{table}

